Dependency-Aware Release Planning for Software Projects using Fuzzy Graphs and Integer Programming

Software Release Planning (SRP) is to find, for the software, a subset of the requirements with the highest value while respecting the budget. The value of a requirement however may, to various degrees, depend on selecting or ignoring other requirements. However, existing SRP models ignore either Value-Related Dependencies altogether or the strengths of those dependencies even if they consider them. This paper presents an Integer Programming model for software release planning, which considers the variances of strengths of positive and negative value-related dependencies among software requirements. To capture the imprecision associated with strengths of value-related dependencies we have made use of the algebraic structure of fuzzy graphs. We have further, contributed a scalable technique for automated identification of value-related dependencies based on user preferences for software requirements. The validity of the work is verified through simulations.

==> table_ex_overall_influence.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.9\textwidth }{!}{\begin{tabular}{cccccc}
  \toprule[1.5pt]
  \head{$OI_{i,j}=\rho_{i,j}^{+\infty}-\rho_{i,j}^{-\infty}$} & \head{$r_1$} & \head{$r_2$} & \head{$r_3$} & \head{$r_4$} & \head{$r_5$}\\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $r_1$ & $0.0-0.0=0.0$ & $0.4-0.0=0.0$ & $0.2-0.3=-0.1$ & $0.3-0.0=0.3$ & $0.0-0.5=-0.5$\\
  $r_2$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.2-0.0=0.2$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_3$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_4$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_5$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  \bottomrule[1.5pt]
\end{tabular}}



==> table_ex_overall_strengths.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.7\textwidth }{!}{\begin{tabular}{cccccc}
  \toprule[1.5pt]
  \head{$OI_{i,j}=\rho_{i,j}^{+\infty}-\rho_{i,j}^{-\infty}$} & \head{$r_1$} & \head{$r_2$} & \head{$r_3$} & \head{$r_4$} & \head{$r_5$}\\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $r_1$ & $0.0/0.0$ & $0.4/0.0$ & $0.2/0.3$ & $0.3/0.0$ & $0.0/0.5$\\
  $r_2$ & $0.0/0.0$ & $0.0/0.0$ & $0.2/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  $r_3$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0$ & $0.0/0.0$ \\
  $r_4$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  $r_5$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  \bottomrule[1.5pt]
\end{tabular}}


